A Volume-Limited Survey of mCP Stars Within 100pc I: Fundamental Parameters and Chemical Abundances

We present the first results of a volume-limited survey of main sequence (MS) magnetic chemically peculiar (mCP) stars. The sample consists of all identified intermediate-mass MS stars (mCP and non-mCP) within a heliocentric distance of $100\,{\rm pc}$ as determined using Hipparcos parallaxes. The two populations are compared in order to determine the unique properties that allow a small fraction of MS stars with masses $\gtrsim1.4\,M_\odot$ to host strong, large scale magnetic fields. A total of 52 confirmed mCP stars are identified using published magnetic, spectroscopic, and photometric observations along with archived and newly obtained spectropolarimetric (Stokes $V$) observations. We derive the fundamental parameters (effective temperatures, luminosities, masses, and evolutionary states) of the mCP and non-mCP populations using homogeneous analyses. A detailed analysis of the mCP stars is performed using the {\sc llmodels} code, which allows observed spectral energy distributions to be modeled while incorporating chemical peculiarities and magnetic fields. The surface gravities and mean chemical abundances are derived by modelling averaged spectra using the {\sc gssp} and {\sc zeeman} spectral synthesis codes. Masses and stellar ages are derived using modern, densely calculated evolutionary model grids. We confirm a number of previously reported evolutionary properties associated with mCP stars including a conspicuously high incidence of middle-aged MS stars with respect to the non-mCP subsample; the incidence of mCP stars is found to sharply increase with mass from $0.3$~per~cent at $1.5\,M_\odot$ to $\approx11$~per~cent at $3.8\,M_\odot$. Finally, we identify clear trends in the mean photospheric chemical abundances with stellar age.

==> tbl_fund_tbl_short.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{center}
\begin{longtable}{@{\extracolsep{\fill}}l c c c c c c r@{\extracolsep{\fill}}}
\caption[asdf]{Derived fundamental parameters for the 52 confirmed mCP stars and 3 candidate mCP 
	stars (HD~15717, HD~32576, and HD~217831) in the sample. Columns (1) through (4) list parameters 
	derived from the spectroscopic and photometric observations. Columns (5) through (8) list parameters 
	derived using the evolutionary models generated by \citet{Mowlavi2012} and 
	\citet{Ekstrom2012}.} \label{tbl:fund_tbl} \\
	
\hline
\hline
\noalign{\vskip0.5mm}
	HD  & $T_{\rm eff}\,({\rm K})$ & $R\,(R_\odot)$ & $\log{L/L_\odot}$ & $M\,(M_\odot)$ & $\log{(g)}_{\rm HRD}$ & $\log{t/{\rm Gyrs}}$ & $\tau$ \\
	(1) & (2)                      & (3)            & (4)               & (5)            & (6)                   & (7)                  & (8)    \\
\noalign{\vskip0.5mm}
\hline
\noalign{\vskip0.5mm}
\endfirsthead

\multicolumn{8}{l}{continued from previous page}\\
\hline
\hline
\noalign{\vskip0.5mm}
	HD  & $T_{\rm eff}\,({\rm K})$ & $R\,(R_\odot)$ & $\log{L/L_\odot}$ & $M\,(M_\odot)$ & $\log{(g)}_{\rm HRD}$ & $\log{t/{\rm Gyrs}}$ & $\tau$ \\
	(1) & (2)                      & (3)            & (4)               & (5)            & (6)                   & (7)                  & (8)    \\
\noalign{\vskip0.5mm}
\hline	
\noalign{\vskip0.5mm}
\endhead

\noalign{\vskip0.5mm}\hline
\multicolumn{8}{l}{continued on next page}\\
\endfoot

\noalign{\vskip0.5mm}\hline
\endlastfoot

3980   &    $8620\pm420$ &   $1.85\pm0.19$ &   $1.23\pm0.04$ &    $1.96_{-0.21}^{+0.13}$ &             $4.20\pm0.10$ &    $8.67_{-0.70}^{+0.30}$ &    $0.41_{-0.33}^{+0.35}$ \\
11502  &   $10120\pm650$ &   $1.86\pm0.31$ &   $1.52\pm0.09$ &    $2.36_{-0.29}^{+0.17}$ &    $4.27_{-0.15}^{+0.10}$ &    $8.18_{-0.76}^{+0.52}$ &    $0.23_{-0.19}^{+0.45}$ \\
12446  &   $10000\pm710$ &   $2.66\pm0.45$ &   $1.80\pm0.08$ &    $2.64_{-0.28}^{+0.21}$ &             $4.01\pm0.14$ &    $8.52_{-0.27}^{+0.16}$ &    $0.68_{-0.29}^{+0.22}$ \\
15089  &    $8530\pm270$ &   $2.06\pm0.16$ &   $1.30\pm0.04$ &    $2.02_{-0.22}^{+0.14}$ &    $4.12_{-0.08}^{+0.07}$ &    $8.76_{-0.27}^{+0.20}$ &    $0.56_{-0.24}^{+0.27}$ \\
15144  &    $8510\pm240$ &   $2.07\pm0.17$ &   $1.31\pm0.06$ &    $2.02_{-0.22}^{+0.15}$ &    $4.11_{-0.08}^{+0.07}$ &    $8.77_{-0.24}^{+0.19}$ &    $0.57_{-0.23}^{+0.26}$ \\
15717  &   $6850\pm1020$ &   $1.70\pm0.22$ &   $0.76\pm0.20$ &    $1.49_{-0.24}^{+0.12}$ &    $4.15_{-0.13}^{+0.11}$ &    $9.17_{-0.50}^{+0.35}$ &    $0.63_{-0.42}^{+0.49}$ \\
18296  &   $10010\pm750$ &   $2.89\pm0.46$ &   $1.88\pm0.05$ &    $2.74_{-0.27}^{+0.19}$ &             $3.95\pm0.14$ &    $8.52_{-0.21}^{+0.13}$ &    $0.74_{-0.24}^{+0.20}$ \\
24712  &    $7150\pm170$ &   $1.80\pm0.11$ &   $0.88\pm0.03$ &    $1.60_{-0.16}^{+0.10}$ &    $4.13_{-0.07}^{+0.06}$ &    $9.06_{-0.22}^{+0.20}$ &    $0.60_{-0.25}^{+0.30}$ \\
27309  &   $11290\pm660$ &   $2.30\pm0.31$ &   $1.89\pm0.05$ &    $2.87_{-0.31}^{+0.20}$ &    $4.17_{-0.13}^{+0.11}$ &    $8.21_{-0.73}^{+0.30}$ &             $0.41\pm0.33$ \\
29305  &   $11810\pm450$ &   $3.19\pm0.28$ &   $2.25\pm0.04$ &    $3.41_{-0.32}^{+0.09}$ &    $3.96_{-0.08}^{+0.07}$ &    $8.26_{-0.08}^{+0.13}$ &    $0.72_{-0.12}^{+0.18}$ \\
32576  &    $8180\pm240$ &   $1.76\pm0.10$ &   $1.10\pm0.14$ &    $1.83_{-0.20}^{+0.13}$ &    $4.21_{-0.07}^{+0.05}$ &    $8.74_{-0.39}^{+0.28}$ &    $0.40_{-0.24}^{+0.34}$ \\
38823  &    $7750\pm360$ &   $1.54\pm0.23$ &   $0.88\pm0.10$ &    $1.65_{-0.20}^{+0.12}$ &    $4.28_{-0.13}^{+0.07}$ &    $8.58_{-0.76}^{+0.56}$ &    $0.21_{-0.17}^{+0.52}$ \\
40312  &   $10220\pm360$ &   $4.68\pm0.34$ &   $2.33\pm0.02$ &    $3.24_{-0.25}^{+0.23}$ &    $3.61_{-0.07}^{+0.08}$ &    $8.46_{-0.10}^{+0.02}$ &    $1.00_{-0.06}^{+0.01}$ \\
49976  &    $9460\pm380$ &   $1.95\pm0.20$ &   $1.44\pm0.06$ &    $2.22_{-0.25}^{+0.15}$ &    $4.20_{-0.10}^{+0.08}$ &    $8.48_{-0.62}^{+0.32}$ &    $0.38_{-0.29}^{+0.35}$ \\
54118  &   $10910\pm350$ &   $2.61\pm0.24$ &   $1.94\pm0.06$ &    $2.89_{-0.29}^{+0.20}$ &             $4.07\pm0.09$ &    $8.36_{-0.22}^{+0.17}$ &    $0.60_{-0.22}^{+0.23}$ \\
56022  &    $9660\pm240$ &   $2.00\pm0.10$ &   $1.50\pm0.02$ &    $2.29_{-0.24}^{+0.15}$ &    $4.20_{-0.07}^{+0.06}$ &    $8.45_{-0.43}^{+0.29}$ &    $0.39_{-0.24}^{+0.32}$ \\
62140  &    $7740\pm460$ &   $2.32\pm0.33$ &   $1.24\pm0.08$ &    $1.92_{-0.25}^{+0.14}$ &             $3.99\pm0.13$ &             $8.95\pm0.19$ &             $0.74\pm0.24$ \\
64486  &   $10490\pm460$ &   $2.61\pm0.28$ &   $1.88\pm0.05$ &    $2.77_{-0.28}^{+0.19}$ &    $4.05_{-0.10}^{+0.09}$ &    $8.43_{-0.23}^{+0.16}$ &    $0.63_{-0.24}^{+0.22}$ \\
65339  &    $8520\pm320$ &   $2.43\pm0.23$ &   $1.45\pm0.06$ &    $2.16_{-0.22}^{+0.15}$ &             $4.00\pm0.09$ &    $8.79_{-0.15}^{+0.13}$ &             $0.71\pm0.19$ \\
72968  &    $9310\pm490$ &   $2.32\pm0.26$ &   $1.56\pm0.05$ &    $2.32_{-0.25}^{+0.16}$ &             $4.07\pm0.11$ &    $8.63_{-0.28}^{+0.18}$ &    $0.60_{-0.27}^{+0.25}$ \\
74067  &   $10190\pm380$ &   $2.44\pm0.25$ &   $1.76\pm0.07$ &    $2.62_{-0.28}^{+0.18}$ &             $4.08\pm0.09$ &    $8.47_{-0.26}^{+0.18}$ &             $0.58\pm0.25$ \\
83368  &    $7660\pm220$ &   $2.00\pm0.15$ &   $1.09\pm0.04$ &    $1.78_{-0.17}^{+0.12}$ &    $4.09_{-0.08}^{+0.07}$ &    $8.97_{-0.20}^{+0.15}$ &    $0.62_{-0.21}^{+0.28}$ \\
96616  &    $9180\pm400$ &   $2.85\pm0.28$ &   $1.72\pm0.04$ &    $2.48_{-0.24}^{+0.16}$ &    $3.93_{-0.10}^{+0.09}$ &             $8.66\pm0.12$ &             $0.78\pm0.17$ \\
103192 &   $11750\pm380$ &   $3.86\pm0.38$ &   $2.41\pm0.07$ &    $3.65_{-0.53}^{+0.08}$ &    $3.83_{-0.11}^{+0.06}$ &    $8.25_{-0.03}^{+0.13}$ &    $0.89_{-0.05}^{+0.09}$ \\
108662 &    $9740\pm460$ &   $2.11\pm0.21$ &   $1.56\pm0.04$ &    $2.36_{-0.25}^{+0.16}$ &             $4.16\pm0.10$ &    $8.49_{-0.48}^{+0.27}$ &    $0.46_{-0.29}^{+0.32}$ \\
108945 &    $8670\pm230$ &   $2.64\pm0.16$ &   $1.55\pm0.03$ &    $2.27_{-0.22}^{+0.14}$ &    $3.95_{-0.07}^{+0.06}$ &             $8.76\pm0.10$ &    $0.76_{-0.14}^{+0.17}$ \\
109026 &   $11800\pm900$ &   $2.68\pm0.82$ &   $2.10\pm0.21$ &    $3.19_{-0.40}^{+0.29}$ &    $4.08_{-0.22}^{+0.20}$ &    $8.22_{-0.72}^{+0.21}$ &    $0.56_{-0.46}^{+0.31}$ \\
112185 &    $9350\pm330$ &   $3.99\pm0.28$ &   $2.04\pm0.02$ &    $2.94_{-0.41}^{+0.15}$ &    $3.70_{-0.10}^{+0.07}$ &    $8.54_{-0.05}^{+0.12}$ &    $0.94_{-0.08}^{+0.07}$ \\
112413 &   $11320\pm600$ &   $2.52\pm0.31$ &   $1.97\pm0.07$ &    $2.97_{-0.32}^{+0.22}$ &             $4.11\pm0.11$ &    $8.28_{-0.43}^{+0.22}$ &    $0.53_{-0.31}^{+0.28}$ \\
117025 &    $8590\pm470$ &   $2.12\pm0.25$ &   $1.34\pm0.04$ &    $2.06_{-0.21}^{+0.14}$ &             $4.10\pm0.11$ &    $8.76_{-0.32}^{+0.19}$ &    $0.58_{-0.29}^{+0.27}$ \\
118022 &    $9440\pm270$ &   $1.96\pm0.11$ &   $1.44\pm0.02$ &    $2.22_{-0.24}^{+0.14}$ &    $4.20_{-0.07}^{+0.06}$ &    $8.50_{-0.45}^{+0.30}$ &    $0.39_{-0.25}^{+0.32}$ \\
119213 &    $8620\pm470$ &   $1.99\pm0.23$ &   $1.29\pm0.04$ &    $2.02_{-0.22}^{+0.14}$ &             $4.14\pm0.11$ &    $8.73_{-0.43}^{+0.23}$ &             $0.51\pm0.31$ \\
120198 &    $9740\pm560$ &   $2.14\pm0.26$ &   $1.57\pm0.04$ &    $2.37_{-0.25}^{+0.17}$ &    $4.15_{-0.12}^{+0.11}$ &    $8.50_{-0.54}^{+0.25}$ &    $0.47_{-0.33}^{+0.31}$ \\
124224 &   $12260\pm480$ &   $2.05\pm0.19$ &   $1.93\pm0.04$ &    $3.05_{-0.33}^{+0.14}$ &    $4.30_{-0.10}^{+0.05}$ &    $7.63_{-0.51}^{+0.69}$ &    $0.13_{-0.09}^{+0.42}$ \\
128898 &    $7760\pm230$ &   $1.85\pm0.11$ &   $1.05\pm0.01$ &    $1.76_{-0.17}^{+0.12}$ &    $4.15_{-0.07}^{+0.06}$ &    $8.92_{-0.30}^{+0.20}$ &    $0.53_{-0.25}^{+0.33}$ \\
130559 &    $9120\pm420$ &   $2.30\pm0.25$ &   $1.52\pm0.05$ &    $2.26_{-0.23}^{+0.16}$ &             $4.07\pm0.10$ &    $8.67_{-0.26}^{+0.17}$ &    $0.62_{-0.26}^{+0.25}$ \\
137909 &    $7540\pm420$ &   $3.15\pm0.37$ &   $1.46\pm0.04$ &    $2.14_{-0.35}^{+0.13}$ &    $3.77_{-0.14}^{+0.11}$ &    $8.91_{-0.07}^{+0.16}$ &    $0.92_{-0.13}^{+0.10}$ \\
137949 &    $7370\pm270$ &   $2.16\pm0.24$ &   $1.09\pm0.07$ &    $1.77_{-0.28}^{+0.13}$ &    $4.02_{-0.12}^{+0.08}$ &    $9.04_{-0.15}^{+0.25}$ &    $0.72_{-0.19}^{+0.34}$ \\
140160 &    $9030\pm230$ &   $2.17\pm0.15$ &   $1.45\pm0.04$ &    $2.19_{-0.23}^{+0.15}$ &    $4.11_{-0.08}^{+0.06}$ &    $8.67_{-0.22}^{+0.19}$ &    $0.56_{-0.21}^{+0.26}$ \\
140728 &    $9730\pm550$ &   $2.44\pm0.30$ &   $1.69\pm0.03$ &    $2.49_{-0.25}^{+0.17}$ &    $4.06_{-0.12}^{+0.10}$ &    $8.56_{-0.27}^{+0.17}$ &    $0.62_{-0.26}^{+0.25}$ \\
148112 &    $9170\pm390$ &   $3.34\pm0.33$ &   $1.85\pm0.06$ &    $2.66_{-0.41}^{+0.16}$ &    $3.81_{-0.11}^{+0.09}$ &    $8.63_{-0.08}^{+0.17}$ &    $0.87_{-0.13}^{+0.14}$ \\
148898 &    $8150\pm250$ &   $2.97\pm0.19$ &   $1.54\pm0.02$ &    $2.25_{-0.35}^{+0.13}$ &    $3.85_{-0.10}^{+0.06}$ &    $8.82_{-0.07}^{+0.18}$ &    $0.86_{-0.11}^{+0.15}$ \\
151199 &    $8620\pm390$ &   $2.06\pm0.20$ &   $1.32\pm0.04$ &    $2.04_{-0.21}^{+0.14}$ &             $4.12\pm0.10$ &    $8.74_{-0.34}^{+0.21}$ &             $0.55\pm0.28$ \\
152107 &    $8840\pm190$ &   $2.30\pm0.11$ &   $1.47\pm0.03$ &    $2.19_{-0.22}^{+0.14}$ &    $4.06_{-0.06}^{+0.05}$ &             $8.72\pm0.16$ &    $0.64_{-0.18}^{+0.22}$ \\
170000 &   $11630\pm110$ &   $3.73\pm0.14$ &   $2.36\pm0.04$ &    $3.56_{-0.49}^{+0.04}$ &    $3.85_{-0.07}^{+0.03}$ &    $8.27_{-0.01}^{+0.12}$ &    $0.88_{-0.03}^{+0.09}$ \\
176232 &    $7440\pm370$ &   $2.69\pm0.30$ &   $1.30\pm0.04$ &    $1.96_{-0.40}^{+0.12}$ &    $3.87_{-0.12}^{+0.09}$ &    $8.99_{-0.09}^{+0.24}$ &    $0.86_{-0.15}^{+0.21}$ \\
187474 &    $9900\pm400$ &   $2.56\pm0.35$ &   $1.76\pm0.09$ &    $2.58_{-0.27}^{+0.20}$ &    $4.03_{-0.11}^{+0.10}$ &    $8.53_{-0.21}^{+0.15}$ &    $0.65_{-0.24}^{+0.23}$ \\
188041 &    $8520\pm340$ &   $2.32\pm0.19$ &   $1.41\pm0.04$ &    $2.11_{-0.22}^{+0.14}$ &             $4.03\pm0.08$ &    $8.79_{-0.18}^{+0.15}$ &             $0.67\pm0.21$ \\
201601 &    $7570\pm170$ &   $2.07\pm0.12$ &   $1.10\pm0.03$ &    $1.78_{-0.17}^{+0.12}$ &    $4.06_{-0.07}^{+0.06}$ &    $9.00_{-0.15}^{+0.13}$ &    $0.67_{-0.18}^{+0.25}$ \\
203006 &    $9240\pm480$ &   $2.35\pm0.34$ &   $1.56\pm0.09$ &    $2.32_{-0.26}^{+0.18}$ &             $4.06\pm0.12$ &    $8.64_{-0.28}^{+0.17}$ &    $0.62_{-0.28}^{+0.25}$ \\
217522 &    $6520\pm280$ &   $1.92\pm0.28$ &   $0.78\pm0.09$ &    $1.48_{-0.27}^{+0.13}$ &    $4.04_{-0.16}^{+0.10}$ &    $9.32_{-0.17}^{+0.30}$ &    $0.86_{-0.28}^{+0.49}$ \\
217831 &   $6900\pm1350$ &   $2.58\pm0.31$ &   $1.13\pm0.14$ &    $1.79_{-0.31}^{+0.12}$ &    $3.87_{-0.14}^{+0.12}$ &    $9.11_{-0.11}^{+0.22}$ &    $0.88_{-0.18}^{+0.23}$ \\
220825 &    $9180\pm370$ &   $1.73\pm0.14$ &   $1.28\pm0.03$ &    $2.06_{-0.22}^{+0.11}$ &    $4.27_{-0.09}^{+0.07}$ &    $8.36_{-0.80}^{+0.48}$ &    $0.23_{-0.20}^{+0.40}$ \\
221760 &    $8470\pm230$ &   $3.62\pm0.27$ &   $1.78\pm0.05$ &    $2.55_{-0.39}^{+0.15}$ &    $3.73_{-0.10}^{+0.07}$ &    $8.71_{-0.05}^{+0.14}$ &             $0.94\pm0.09$ \\
223640 &   $12240\pm440$ &   $2.30\pm0.22$ &   $2.03\pm0.05$ &    $3.17_{-0.34}^{+0.20}$ &    $4.21_{-0.10}^{+0.07}$ &    $7.98_{-0.74}^{+0.37}$ &    $0.32_{-0.26}^{+0.35}$ \\
\end{longtable}
\end{center}
\renewcommand{\arraystretch}{1.0}
